Social Simulacra: Creating Populated Prototypes for Social Computing Systems

Social computing prototypes probe the social behaviors that may arise in an envisioned system design. This prototyping practice is currently limited to recruiting small groups of people. Unfortunately, many challenges do not arise until a system is populated at a larger scale. Can a designer understand how a social system might behave when populated, and make adjustments to the design before the system falls prey to such challenges? We introduce social simulacra, a prototyping technique that generates a breadth of realistic social interactions that may emerge when a social computing system is populated. Social simulacra take as input the designer's description of a community's design -- goal, rules, and member personas -- and produce as output an instance of that design with simulated behavior, including posts, replies, and anti-social behaviors. We demonstrate that social simulacra shift the behaviors that they generate appropriately in response to design changes, and that they enable exploration of "what if?" scenarios where community members or moderators intervene. To power social simulacra, we contribute techniques for prompting a large language model to generate thousands of distinct community members and their social interactions with each other; these techniques are enabled by the observation that large language models' training data already includes a wide variety of positive and negative behavior on social media platforms. In evaluations, we show that participants are often unable to distinguish social simulacra from actual community behavior and that social computing designers successfully refine their social computing designs when using social simulacra.

==> content/discussion_old.tex <==
\section{DISCUSSION}
In this section, we reflect on social simulacra's contributions, ethical considerations, limitations, and opportunities for future work. 


\subsection{Limitations and Future Work}
We believe that our implementation of a Social Simulacra, SimReddit presents a step forward in approaches for designing and prototyping social platforms. However, there are still several limitations to consider, as well as promising avenues for further work.

Limits of Social Simulacra. SimReddit cannot simulate the one way a social platform will turn out. However, Social Simulacra will never have this ability, not due to some inherent deficiency, but because social media outcomes are non-deterministic and incredibly dependent on initial conditions. Multiple real-world instantiations of the same social system could have different results, due to the diversity and complexity of human behavior; no simulation will be able to give a definitive answer as to the resulting state of a new community. 

Despite this fundamental limitation, we believe that Social Simulacra, and SimReddit itself, show promise for helping designers evaluate and iterate on their designs for social computing systems. We focus our efforts on opening the designers up to a diverse set of possibilities - of topic and behavior - rather than guaranteeing them a certain outcome (which does not exist). 

\subsubsection{Limits of SimReddit}
Some features were not possible within SimReddit, but are possible in future Social Simulacra possibilities, depending on advancements in foundation models. For example, if LLM attention improves, we could consider increasing the context from a single conversation to the entire community. It is well known that posts within a community can influence future posting behavior, so given suitable technical capabilities, this relationship could be implemented within Social Simulacra. This functionality would allow designers to ask higher-level questions about the trajectory of the community- perhaps experimenting with seeding the platform with content. Additionally, with longer contexts, the “personas” that we use could be more consistent and complex, involving interpersonal relationships that impact and are impacted by the content generated.

Another opportunity for expansion is across content types. Currently, our tool is text-only, but in the future, we can imagine opening up the types of content generated, thereby allowing the kinds of multimodal posts (for example, text and video) that are common on most social platforms today. Such an advancement would greatly increase the insights available to designers; many abuse types occur across a mix of text, photo, video, and more.

\subsubsection{Other Possibilities} 
Within this project, we considered adding functionality for non-text engagement: an instantiation of audience approval/disapproval like retweets, upvotes, likes, shares, etc. We chose not to include this feature in SimReddit because our tool was not operating at the scale of generation that would produce usable insights from these engagement measures. Particularly, we note the opportunity for addressing design questions around possible effects of content algorithms by simulating user behavior around engagement features. Additionally, with advancements in foundation model attention and then potentially an implementation of community wide-contexts, we could simulate much larger social effects that could help designers understand the tradeoffs of different algorithm types, engagement affordances, and more. We also considered implementing opportunities for moderation to be simulated; among these was a rule classification system to replicate auto-moderation systems and remove content classified as violating rules. 


\subsection{Ethical considerations}
Beyond the limitations of the functionality of Social Simulacra, we believe there are further ethical implications to consider.

\subsubsection{Antisocial content generation} Concerns have been raised about the problematic and discriminatory generations of foundation models []. Within our prototyping use-case, this behavior is an asset to our tool; by replicating the bigoted and hateful behavior that has occurred online in the past, we allow designers to anticipate this behavior in their own contexts so they can design to account for these problems. For this reason, it is very possible that SimReddit will expose designers to upsetting or triggering content. However, designers are already at risk of seeing such content in their deployed community, and in that situation, users would also be exposed.

Nonetheless, the antisocial content that foundation models can generate poses problems in the case of their misuse. Already, bad actors can use foundation models to generate content for nefarious purposes. Language generation without significant use or rate restrictions can be used for astroturfing, large-scale harassment attacks, propaganda, and more. These harassment types are also possible without use of a LLM; these models just make it easier, faster, and more scalable. 

We do not believe that most of the prompting improvements we have made are useful to the aforementioned bad actors. Our prompting innovations focused on creating a diverse set of content that made sense in the context of a particular community, which is contrary to the aims of most malicious actors who are seeking to generate a very particular content type at scale. We also came up with techniques for generating content influenced by rules, and that incorporated quotations, neither of which are particularly relevant to many of the antisocial use cases we can imagine. Use of our tool would not improve scale very well for the aforementioned malicious uses, since it would require adaptation to a particular use-case as well as human filtering to get consistently viable results. Since the end result could also be achieved by more manual use of a LLM, we are less concerned about the potential for harmful content created by our tool; it does not contribute much utility that we can imagine to said malicious users. 

However, we do recognize that contextualized antisocial behavior may be useful to bad actors, especially in the context of sowing dissent or spreading disinformation on a platform made up of smaller, niche communities. For this reason, we will withhold our code for [X amount of time] from the general public, upon which we will re-evaluate the risk associated with code release. 

\subsubsection{Negative Impact on Design} 
As established earlier, our prototyping tool is imperfect, which means it could mislead designers and cause them to apply those misconceptions to their design. We try to mitigate this by presenting many possibilities to the designers who use our tool; in seeing multiple possible results, the perceived certainty of any one is lessened.

We also rely partially on the intuition of our designers: it falls on them to discern what content and behavior is possible, as well as to imagine design changes that will discourage the undesired behavior and encourage the behaviors they want on their platform. The latter is somewhat implicit in their job title, and one we feel is quite reasonable to outsource to the designers. The first, however, is perhaps a less reasonable requirement; are designers capable of discerning what generations are relevant or likely? Based on our user study, we do believe that social platform designers are often capable of discerning realistic content in their community. They also connect unexpected content to the community and its design, areas in which they are knowledgeable, to generate theories about what problems they need to address, rather than creating individual rules based on each problematic comment they see. These strategies mitigate the risk of designers worsening their designs in response to faulty generations.

We also acknowledge the possibility that designers could use our tool to generate a non-comprehensive list of possible issues, and then only address items on said list; however, such a list would still have better coverage than current strategies. Theoretically, any prototyping tool could be abused in the hands of a user who wants to skip truly evaluating their creation. We hope that the focus of our tool on exploring different possibilities will spark insights about areas for improvement, without creating a sense that said exploration is ever truly complete.

We also make some of the simulation’s assumptions visible to the designer via the input fields. The user is aware of what inputs the tool accepts, and is therefore aware that more complex characteristics of a community (beyond goal, rules, and population personas) do not play a role in the generated content. Personas are an imperfect design tool, but they are useful within our system to increase the variability of posts and comments, so we make their inclusion clear to the user by requiring them to input the “seed” personas through which more are generated.



\subsection{Implications for Social Platform Design}
One implication of this work on design practices is a turn towards proactive, instead of reactive, design. Many of our interviewees commented on the negatives of only fixing mistakes they already caused harm, and wished for opportunities to evaluate their designs ahead of deployment. They noticed flaws in the design largely by recognizing instances of harm to users, and then backtracking to find the underlying cause or coming up with a missing mitigation strategy. Such reactive strategies thereby require harm to users and communities as a condition for improvement; prototyping tools like ours can minimize the need for these strategies. We hope that our contribution can help prompt development of further tools and techniques that facilitate reflection on designs for social computing systems prior to affecting real people.

An additional possibility for this work is to be used in educational contexts. Both designers and moderators can benefit from exploring the variety of ways that their users and community may behave. Our interview participants remarked on their uncertainty about (a) how to respond to users as a moderator or (b) the proper ways to enforce particular rules. This tool, or similar ones, can also allow moderators to explore possible reactions to their micro-interventions, like responding in a specific way to a misbehaving user. In anticipating different reactions, moderators can prepare different responses and sanction methods, rather than being caught unawares in the moment. Prototyping tools like ours allow for training and exploration throughout the range of possible responses, rather than through trial and error with actual users or a limited set of contrived, pre-written examples. Some moderator learning resources exist but they are focused on how to use moderating tools (Twitch, Reddit), or at least address general situations (Discord Moderator Academy, other examples), without the context of a particular community.


==> content/discussion_old_2.tex <==
\section{DISCUSSION}
In this section, we reflect on social simulacra's contributions, ethical considerations, limitations, and opportunities for future work. 

\subsection{Designing With Social Simulacra}
As defined in the paper, social simulacra 



I would encourage a first short section of discussion to reflect on: why did this work? What are social simulacra allowing designers to reflect on? If we view design as an iterative reflective loop, what feedback are they getting that's helpful? What feedback isn't helpful? And what feedback would be helpful, but social simulacra can't give them yet?

--> how does this change the design process? What could we not do in the past that this enables? 

"We have to remember, right now, there really is no way to do this shit... We usually use crowdworkers but you are seriously mistaken if you think they will offer you something realisitc just because they are people" 

\subsubsection{Disentangling the implementation and the approach}


What can we do (even if we didn't do in this work) say with GPT-3? 
posts and replies
interactions (likes, RTs, etc)
moderation behaviors
ranking outcomes
&etc

Newer models... might even let us do more than this! 

\subsubsection{Dangers of mis-leading designers?? }
False negative, 
people optimizing for social simulacra...


\subsection{Ethical Considerations}
Our approach introduces 

\subsubsection{Antisocial content generation}

\subsubsection{Exposing harmful content to the designers}
Social simulacra may expose designers to potentially harmful and upsetting content. To a large extent, this is side-effect of our approach as its goal is to present a wide array of possibilities, both good and bad, that could take place in the designer's community. We argue that 

 basically accepting this risk of harm to the designer because the overall harm is lower than if both the designer and the users were exposed to harmful content. 

good and bad things that could happen in the designer's community .

Concerns have been raised about the problematic and discriminatory generations of foundation models []. Within our prototyping use-case, this behavior is an asset to our tool; by replicating the bigoted and hateful behavior that has occurred online in the past, we allow designers to anticipate this behavior in their own contexts so they can design to account for these problems. For this reason, it is very possible that SimReddit will expose designers to upsetting or triggering content. However, designers are already at risk of seeing such content in their deployed community, and in that situation, users would also be exposed.


Anti social generation

Exposing people to bad stuff 


\subsection{Future Work}

new models! 
human + simulacra generate? 
interactive simulacra.... 

==> figures/tech_eval.tex <==
\begin{figure}[tb]
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/images/tech_eval.jpg}
  \caption{WhatIf can surface how a conversation might have developed if someone else (e.g., a troll) had responded or intervened (e.g., a moderator).}
  \label{fig: technical eval}
\end{figure}

